Studying Ranking-Incentivized Web Dynamics

The ranking incentives of many authors of Web pages play an important role in the Web dynamics. That is, authors who opt to have their pages highly ranked for queries of interest, often respond to rankings for these queries by manipulating their pages; the goal is to improve the pages' future rankings. Various theoretical aspects of this dynamics have recently been studied using game theory. However, empirical analysis of the dynamics is highly constrained due to lack of publicly available datasets.We present an initial such dataset that is based on TREC's ClueWeb09 dataset. Specifically, we used the WayBack Machine of the Internet Archive to build a document collection that contains past snapshots of ClueWeb documents which are highly ranked by some initial search performed for ClueWeb queries. Temporal analysis of document changes in this dataset reveals that findings recently presented for small-scale controlled ranking competitions between documents' authors also hold for Web data. Specifically, documents' authors tend to mimic the content of documents that were highly ranked in the past, and this practice can result in improved ranking.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> datasetStats.tex <==
\begin{table}
  \caption{\label{tab:stats} Dataset statistics.}
  \begin{tabular}{lcl}
    \toprule
    \# of unique documents in the base set & 9,986\\
    \# of documents in the base set with at least one  & 7,424\\
    Mean Snapshots Per Covered Document & 5.42\\
    Median Snapshots Per Covered Document  & 4\\
    Max Snapshots For Covered Document  & 45\\
  \bottomrule
\end{tabular}
\end{table}


==> macros.tex <==
%%% editing macros
\renewcommand{\comment}[1]{{\bf {\small !!--#1--!!}}}
\newcommand{\omt}[1]{}
\newcommand{\firstmention}[1]{{\bf #1}}
\newcommand{\myparagraph}[1]{\vspace{0.3\baselineskip}\noindent{\textbf{#1}}.~}


\newcommand{\topical}{Sub-Topic\xspace}
\newcommand{\nonRelevant}{Not-Relevant\xspace}
\newcommand{\docLength}{Doc-Length\xspace}
\newcommand{\incQueryTerms}{Query-Terms\xspace}
\newcommand{\herding}{Herding\xspace}
\newcommand{\biasing}{Biasing\xspace}
\newcommand{\lmart}{LambdaMART\xspace}
\newcommand{\RM}{RM1\xspace}
\newcommand{\control}{Control\xspace}
\newcommand{\group}[1]{Group{#1}\xspace}
\newcommand{\stb}{STB\xspace}
\newcommand{\sth}{STH\xspace}
\newcommand{\nrh}{NRH\xspace}
\newcommand{\dlh}{DLH\xspace}
\newcommand{\qth}{QTH\xspace}

%%% basic quantities
\newcommand{\query}{q}
\newcommand{\topic}{T}
\newcommand{\subTopicParm}[1]{\topic^{sub}_{#1}}
\newcommand{\subTopic}{\topic^{sub}}
\newcommand{\doc}{d}
\newcommand{\corpus}{\mathcal{D}}
\newcommand{\initTag}{{\rm init}}
%\newcommand{\topRetGroup}{{\mathcal{D}}^{[\numDoc]}_{\initTag}}
\newcommand{\topRetGroup}{{\mathcal{D}}_{\initTag}}
\newcommand{\topRetGroupParam}[1]{{\mathcal{D}}^{[#1]}_{\initTag}}
\newcommand{\numDoc}{n}
\newcommand{\arbTerm}{w}
\newcommand{\stopList}{L_s}
\newcommand{\numRelDocs}{l}
\newcommand{\minVal}{\alpha}
\newcommand{\clipVal}{\eta}





%%% risk minimization
\newcommand{\model}{\theta}
\newcommand{\simpleConst}{c}
\newcommand{\queryMLE}{\model^{MLE}_{\query}}
\newcommand{\queryModel}{\model_{\query}}
\newcommand{\anchorParm}{\gamma}
\newcommand{\queryModelSingleParam}[1]{\model_{\query;\anchorParm,\numTerms}^{[#1]}}
\newcommand{\queryModelClipped}[1]{\model_{\query;\numTerms}^{clipped[#1]}}
\newcommand{\queryModelParam}[2]{\theta_{\query}^{[#1;#2]}}
\newcommand{\postQueryModel}{\hat{\theta}_{\query}}
\newcommand{\postDocModel}{\hat{\theta}_{\doc}}
\newcommand{\docModel}{\theta_{\doc}}
\newcommand{\userModel}{\mathcal{U}}
\newcommand{\authModel}{\mathcal{A}}
\newcommand{\utilSymbol}{U}
\newcommand{\util}[2]{\utilSymbol(#1|#2)}
\newcommand{\simFn}{Score}
\newcommand{\reward}{\simFn}
\newcommand{\rewardFunc}[2]{\reward(#1,#2)}
\newcommand{\fbModel}{\mathcal{M}}
\newcommand{\arbSet}{\mathcal{S}_{\subTopicParm{i}}}
\newcommand{\precSetSymbol}{\mathcal{P}}
\newcommand{\precSingle}{\rho}
\newcommand{\precSet}[2]{\precSetSymbol(#1;#2)}
\newcommand{\powSet}{2^{\relDocSet}\setminus \emptyset}
\newcommand{\weight}{w}
\newcommand{\fFunc}{f}
\newcommand{\hFunc}{h}
\newcommand{\relDocSet}{\mathcal{D}_{r}}
\newcommand{\relDocSubset}{D_{r}^{'}}
\newcommand{\nonRelDocSet}{S_{nr}}
\newcommand{\feedbackSetFull}{{\mathcal{F}}^{[\numFB]}}
\newcommand{\feedbackSet}{\mathcal{F}}
\newcommand{\numFB}{k}
\newcommand{\setSize}[1]{|{#1}|}

%%% feature functions
\newcommand{\ent}{ENT\xspace}
\newcommand{\swOne}{SW1\xspace}
\newcommand{\swTwo}{SW2\xspace}
\newcommand{\coh}{Coherence\xspace}
\newcommand{\minPrec}{MinPrec\xspace}
\newcommand{\precContrib}{PrecContrib\xspace}
\newcommand{\infOne}{InfAP1\xspace}
\newcommand{\infTwo}{InfAP2\xspace}
\newcommand{\infThree}{InfAP3\xspace}
\newcommand{\infFour}{InfAP4\xspace}
\newcommand{\rankParam}[1]{\pi({#1};\topRetGroup)}
\newcommand{\genRanking}{\pi}
\newcommand{\infAP}[1]{\infAPsym(#1)}
\newcommand{\infAPsym}{infAP\xspace}


%%% general math
\newcommand{\set}[1]{\{#1\}}
\newcommand{\definedas}{\stackrel{def}{=}}
\newcommand{\rankEquiv}{\stackrel{rank}{=}}
\newcommand{\kron}[1]{\delta\hspace{-0.2111em}\left[#1\right]}
\newcommand{\kld}[2]{D\left(#1 \; \Big\vert\Big\vert \,\, #2\right)}
\newcommand{\kldSmall}[2]{D\left(#1 \; \vert\vert \,\, #2\right)}
%\newtheorem{definition}{Definition}
\newcommand{\freq}[2]{{\rm tf}(#1 \in #2)}
\newcommand{\wordIndex}{j} 
\newcommand{\entropy}{H}
\newcommand{\crossEnt}{CE}
\newcommand{\assertion}{\psi} %avoid conflict with \numgenerators
%\newcommand{\ce}[2]{\crossEnt\left(#1 \; \Big\vert\Big\vert \,\, #2\right)}
\newcommand{\ce}[2]{\crossEnt(#1 \; \vert\vert \,\, #2)}

%%% probability notation
\newcommand{\prob}{p}
\newcommand{\probhat}{\hat{\prob}}
\newcommand{\modelprob}{\hat{\prob}}
\newcommand{\lmprob}{\modelprob^{LM}}
\newcommand{\ilmprob}{\prob} %for decorating induced probs, if necessary
\newcommand{\ilmprobtil}{\tilde{\prob}}
\newcommand{\baseprob}{\prob}
\newcommand{\condArbP}[3]{\ensuremath{#1(#2 \vert #3)}}
\newcommand{\condP}[2]{\condArbP{\prob}{#1}{#2}}
\newcommand{\estCondP}[2]{\hat{\prob}(#1\vert#2)}
\newcommand{\condPhat}[2]{\hat{\prob}(#1|#2)}
\newcommand{\modelcondP}[2]{\condArbP{\modelprob}{#1}{#2}}
\newcommand{\basecondP}[2]{\condArbP{\baseprob}{#1}{#2}}
\newcommand{\lmcondP}[2]{\condArbP{\lmprob}{#1}{#2}}
\newcommand{\genprob}[2]{\inducedprob{\ilmprob}{#1}{#2}} %text string goes second
\newcommand{\MLE}{MLE\xspace}
\newcommand{\GEN}{GEN\xspace}

%%% induced LMs
\newcommand{\inducedprob}[3]{\ensuremath{#1_{#2}(#3)}}
\newcommand{\inducedlmprob}[2]{\inducedprob{\ilmprob}{#1}{#2}}
\newcommand{\mlprob}[2]{\inducedprob{\ilmprob^{MLE}}{#1}{#2}}
\newcommand{\mlprobTerm}[2]{\inducedprob{\ilmprob^{\,MLE}}{#1}{#2}}
\newcommand{\docinducedlmprob}[1]{\inducedlmprob{\doc}{#1}}
\newcommand{\docinducedlmprobmulti}[1]{\inducedprob{\ilmprob^{Dir}}{\doc}{#1}}
\newcommand{\dirichletParam}{\mu}
\newcommand{\dirichletParamEvalSpecific}{\mu(\evaluationMeasure)}
\newcommand{\dirichletLM}[3]{\inducedprob{\ilmprob^{Dir[#3]}}{#1}{#2}}
\newcommand{\numTerms}{\delta}
\newcommand{\mixLM}[2]{\inducedprob{\ilmprob^{Mix[\mixParam,\numTerms]}}{#1}{#2}}
\newcommand{\mixLMParam}[4]{\inducedprob{\ilmprob^{Mix[#3,#4]}}{#1}{#2}}
\newcommand{\dirichletLMTerm}[3]{\dirichletLM{#1}{#2}{#3}}
\newcommand{\bareMLProb}[1]{\ilmprob^{MLE}_{#1}}
\newcommand{\bareMLProbTerm}[1]{\widetilde{\ilmprob}^{\,MLE}_{#1}}
\newcommand{\bareDirProb}[1]{\ilmprob^{[\dirichletParam]}_{#1}}
\newcommand{\docLengthMax}{\psi}

%%% methods and baselines
\newcommand{\ourAlgSym}{Subsets}
\newcommand{\ourAlg}[1]{\ourAlgSym(#1)}
\newcommand{\ourUAlg}[1]{U\ourAlgSym(#1)}
\newcommand{\ourUUAlg}[1]{U\ourAlgSym(#1)}
\newcommand{\select}[1]{Select(#1)}
\newcommand{\svmRank}{SVM$^{rank}$\xspace}
\newcommand{\relModel}{R\xspace}
\newcommand{\mixModel}{MM\xspace}
\newcommand{\swlm}{SWLM\xspace}
\newcommand{\medmm}{MEDMM\xspace}
\newcommand{\prm}{Passage\xspace}
\newcommand{\predm}{PredictM\xspace}
\newcommand{\svmc}{SVMC\xspace}
\newcommand{\cltr}{ClustLTR\xspace}
\newcommand{\cmrf}{ClustMRF\xspace}
\newcommand{\drift}{ClustDrift\xspace}
\newcommand{\init}{Initial\xspace}

%%% collections
\newcommand{\ap}{AP\xspace}
\newcommand{\robust}{ROBUST\xspace}
\newcommand{\govtwo}{GOV2\xspace}
\newcommand{\clueweb}{ClueWeb\xspace}

%%% metrics
\newcommand{\map}{MAP\xspace}
\newcommand{\precFive}{p@5\xspace}
\newcommand{\ndcg}{NDCG\xspace}
\newcommand{\ablation}{Exclude $\fFunc_i$\xspace}
\newcommand{\single}{Only $\fFunc_i$\xspace}
\newcommand{\rimap}{RI(MAP)\xspace}
\newcommand{\rindcg}{RI(NDCG)\xspace}

%%% significance
\newcommand{\statSymbolAll}{\star}
\newcommand{\statSymbolRM}{r}
\newcommand{\statSymbolSubset}{s}
\newcommand{\statSymbolFB}{m}
\newcommand{\negWeight}{\;\;\,}



\newcommand{\minP}{Min\xspace}
\newcommand{\ameanPrec}{AMean\xspace}
\newcommand{\gmeanPrec}{GMean\xspace}


\newcommand{\hypA}{HypoA\xspace}
\newcommand{\hypB}{HypoB\xspace}
\newcommand{\hypC}{HypoC\xspace}

%\newcommand{\figHeight}{5.6cm}
%\newcommand{\figWidth}{8.7cm}
\newcommand{\figHeight}{5cm}
\newcommand{\figWidth}{8.1cm}

\newcommand{\queryCover}{QueryCover\xspace}
\newcommand{\fracQuery}{FracQuery\xspace}
\newcommand{\pass}{P\xspace}
\newcommand{\act}{A\xspace}
\newcommand{\stba}{\stb-\act}
\newcommand{\stha}{\sth-\act}
\newcommand{\stbp}{\stb-\pass}
\newcommand{\sthp}{\sth-\pass}



==> rankCompetition.tex <==
\section{Rank Competition}
    To understand the incentive of authors in applying the changes we observed, to their web documents, we addressed the document changes over time from a competition point of view, we understand that the goal of authors is to promote their documents as much as possible, but does the strategies we showed authors are using actually work?.
\subsection{Competition Setting}
    We created the following setting to test it, we addressed each time interval as a separate round of a competition, where all documents are competing for the highest rank for their respected query, we analysed several features of the competing documents and observed how these features change over previous rounds for the group of winners in that round (\textbf{W}), the group of documents that received higher (better) ranking in the current round vs previous rounds (\textbf{H}) and the group documents that received lower (worse) in the current round vs previous rounds (\textbf{L}). The features we tested are \textbf{QueryTermsRatio}, \textbf{StopwordsRatio} and \textbf{Entropy} but also the cosine similarity to the previous round winner (\textbf{SimPW}) which had been shown in previous works to be a dominant strategy for authors in controlled document SEO experiments \cite{Raifer17}. The competition was applied on 2 months time intervals, means all document snapshots were aggregated to 2 months time ranges (6 intervals at 2008), if a document had more than one snapshot in this time interval we used only the first snapshot in that interval. Each interval represented a competition round, for each round we ran basic LM retrieval of Dirichlet smoothed language model \cite{Zhai01} with $\mu = 1000$ and negative KL scores \cite{kullback1951} as our ranking function, in each round, for each query q the sub-set of affiliated 50 documents (that had a snapshot in that round) were ranked, each round was set as round 0 at its time, the groups of winners (\textbf{W}), higher ranked documents (\textbf{H}) and lower ranked documents (\textbf{L}) were set according to round 0 rank and previous rounds ranks (-1, -2, -3 and etc), the tested features were calculated for each group in respect to each round 0 and its previous rounds, these features were averaged across all 0 rounds and its respected previous rounds.
    
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{2M_NoLookup_WL_STATS}
  \caption{Mean feature value of documents that won round 0 (\textbf{W}), documents that improved their ranking in round 0 vs previous rounds (\textbf{H}) and documents the received worse ranking in round 0 vs previous rounds (\textbf{L}), x-axis: (minus) number of rounds before round 0}
  \Description{}
\end{figure}

\subsection{Competition Results}
    At Figure 5 we can observe the competition groups and their feature changes over rounds, it is easy to observe that in average, a strategy that is applied by all document authors is to increase similarity to previous winners, this "follow the winner" strategy had been shown before \cite{Raifer17} as a dominant strategy for document authors in controlled experiments, here we verify these findings on the real world web authors behavior, it is easy to see that this strategy also benefits most to the authors that use it more extensively, it is clear that winners in round 0, show larger values in average of similarity to previous winners and a steeper curve of this features increase in the rounds preceding round 0, the steeper increase in SimPW curve in the the rounds preceding round 0 at group H vs group L, indicates that documents that got closer to previous rounds winners had experienced an improvement in their ranking vs authors that applied this strategy in a more moderate way, and received worse their ranking, we also checked the Spearman correlation between ranking in each round vs the SimPW values of each document, the correlation score was \textbf{$0.526$} which indeed indicates on a strong connection between ranking and "follow the winner" strategy. Additionally we can see that QueryTermsRatio is in a moderate upper trend for all documents and as expected, winner documents shows greater values in this feature, empirically this feature is highly correlated with the ranking results of our ranking method, we show that between round -1 and round 0 the W group surpass the L group in this feature average value. It is also visible that winner documents are sowing decreasing trends in Entropy and StopWordsRatio, which indicates it becoming more focused on the queries content, for the Entropy and StopWordsRatio features there is no distinct trend that correlates with one of the W or L groups.
    
    

